Efficient Gaussian Process Classification Using Polya-Gamma Data Augmentation

We propose a scalable stochastic variational approach to GP classification building on Polya-Gamma data augmentation and inducing points. Unlike former approaches, we obtain closed-form updates based on natural gradients that lead to efficient optimization. We evaluate the algorithm on real-world datasets containing up to 11 million data points and demonstrate that it is up to two orders of magnitude faster than the state-of-the-art while being competitive in terms of prediction performance.

==> arXiv18_11 (AAAI version)/new_table.tex <==
\begin{table}[h!]\centering
\begin{adjustbox}{max width=\columnwidth}
\footnotesize
\begin{tabular}{|l|l|l|l|l|}
Dataset & & \textbf{X-GPC} & SVGPC & EPGPC \\\hline
\multirow{1}{*}{aXa} & Error & $ \mathbf{0.17 \pm 0.07} $ & $ \mathbf{0.17 \pm 0.07} $ & $ \mathbf{ 0.17 \pm 0.07 } $\\
$ n=36,974 $ & NLL & $ \mathbf{ 0.29 \pm 0.13 } $ & $ 0.36 \pm 0.13 $ & $ 0.34 \pm 0.13 $\\
$ d=123 $ & Time & $ \mathbf{ 47 \pm 2.2 } $ & $ 451 \pm 7.8 $ & $ 214 \pm 4.8 $\\\hline
\multirow{1}{*}{Bank Market.} & Error & $ 0.14 \pm 0.12 $ & $ \mathbf{0.12 \pm 0.12} $ & $ \mathbf{ 0.12 \pm 0.13 } $\\
$ n=45,211 $ & NLL & $ \mathbf{ 0.27 \pm 0.22 } $ & $ 0.31 \pm 0.26 $ & $ 0.33 \pm 0.20 $\\
$ d=43 $ & Time & $ \mathbf{ 9 \pm 1.5 } $ & $ 205 \pm 6.6 $ & $ 46 \pm 3.5 $\\\hline
\multirow{1}{*}{Click Pred.} & Error & $ \mathbf{ 0.17 \pm 0.00 } $ & $ \mathbf{0.17 \pm 0.00} $ & $ \mathbf{0.17 \pm 0.01} $\\
$ n=399,482 $ & NLL & $ \mathbf{ 0.39 \pm 0.07 } $ & $ 0.46 \pm 0.00 $ & $ 0.46 \pm 0.01 $\\
$ d=12 $ & Time & $ \mathbf{4.5 \pm 1.3} $ & $ 102 \pm 3.0 $ & $ 8.1 \pm 0.45 $\\\hline
\multirow{1}{*}{Cod RNA} & Error & $ \mathbf{ 0.04 \pm 0.00 } $ & $ \mathbf{0.04 \pm 0.00} $ & $ \mathbf{0.04 \pm 0.00} $\\
$ n=343,564 $ & NLL & $ \mathbf{ 0.11 \pm 0.03 } $ & $ 0.13 \pm 0.00 $ & $ 0.12 \pm 0.00 $\\
$ d=8 $ & Time & $ \mathbf{ 3.7 \pm 0.13 } $ & $ 115 \pm 4.3 $ & $ 869 \pm 5.2 $\\\hline
\multirow{1}{*}{Diabetes} & Error & $ \mathbf{0.23 \pm 0.07} $ & $ \mathbf{ 0.23 \pm 0.06 } $ & $ 0.24 \pm 0.06 $\\
$ n=768 $ & NLL & $ \mathbf{ 0.47 \pm 0.11 } $ & $ 0.47 \pm 0.10 $ & $ 0.48 \pm 0.09 $\\
$ d=8 $ & Time & $ 8.8 \pm 0.12 $ & $ 150 \pm 5.1 $ & $ \mathbf{ 8 \pm 0.45 } $\\\hline
\multirow{1}{*}{Electricity} & Error & $ \mathbf{ 0.24 \pm 0.06 } $ & $ 0.26 \pm 0.06 $ & $ 0.26 \pm 0.06 $\\
$ n=45,312 $ & NLL & $ \mathbf{ 0.31 \pm 0.17 } $ & $ 0.53 \pm 0.08 $ & $ 0.53 \pm 0.06 $\\
$ d=8 $ & Time & $ \mathbf{8.2 \pm 0.48} $ & $ 356 \pm 6.9 $ & $ 13.5 \pm 1.50 $\\\hline
\multirow{1}{*}{German} & Error & $ \mathbf{0.25 \pm 0.12} $ & $ \mathbf{ 0.25 \pm 0.11 } $ & $ 0.26 \pm 0.13 $\\
$ n=1,000 $ & NLL & $ \mathbf{ 0.44 \pm 0.17 } $ & $ 0.51 \pm 0.15 $ & $ 0.53 \pm 0.11 $\\
$ d=20 $ & Time & $ 17 \pm 0.42 $ & $ 374 \pm 7.3 $ & $ \mathbf{ 5.2 \pm 0.03 } $\\\hline
\multirow{1}{*}{Higgs} & Error & $ \mathbf{ 0.33 \pm 0.01 } $ & $ 0.45 \pm 0.01 $ & $ 0.38 \pm 0.01 $\\
$ n=11,000,000 $ & NLL & $ \mathbf{ 0.55 \pm 0.13 } $ & $ 0.69 \pm 0.00 $ & $ 0.66 \pm 0.00 $\\
$ d=28 $ & Time & $ \mathbf{ 23 \pm 0.88 } $ & $ 294 \pm 54 $ & $ 8732 \pm 867 $\\\hline
\multirow{1}{*}{IJCNN} & Error & $ 0.03 \pm 0.01 $ & $ 0.06 \pm 0.01 $ & $\mathbf{ 0.02 \pm 0.01} $\\
$ n=141,691 $ & NLL & $ 0.10 \pm 0.03 $ & $ 0.15 \pm 0.07 $ & $ \mathbf{0.09 \pm 0.04} $\\
$ d=22 $ & Time & $ \mathbf{17 \pm 0.44} $ & $ 1033 \pm 45 $ & $ 756 \pm 8.6 $\\\hline
\multirow{1}{*}{Mnist} & Error & $  0.14 \pm 0.01  $ & $ 0.44 \pm 0.13 $ & $ \mathbf{0.12\pm 0.01} $\\
$ n=70,000 $ & NLL & $ \mathbf{ 0.24 \pm 0.10 } $ & $ 0.66 \pm 0.11 $ & $ 0.27 \pm 0.01 $\\
$ d=780 $ & Time & $ \mathbf{200 \pm 5.5} $ & $ 991 \pm 23 $ & $ 806 \pm 5.2 $\\\hline
\multirow{1}{*}{Shuttle} & Error & $ \mathbf{ 0.01 \pm 0.01 } $ & $ \mathbf{0.01 \pm 0.00} $ & $ \mathbf{0.01 \pm 0.01} $\\
$ n=58,000 $ & NLL & $ \mathbf{ 0.07 \pm 0.01 } $ & $ \mathbf{0.07 \pm 0.00} $ & $\mathbf{ 0.07 \pm 0.01 }$\\
$ d=9 $ & Time & $ \mathbf{ 0.01 \pm 0.00 } $ & $ 7.5 \pm 0.7 $ & $ 100 \pm 0.63 $\\\hline
\multirow{1}{*}{SUSY} & Error & $ \mathbf{ 0.21 \pm 0.00 } $ & $ 0.22 \pm 0.00 $ & $ 0.22 \pm 0.00 $\\
$ n=5,000,000 $ & NLL & $ \mathbf{ 0.31 \pm 0.10 } $ & $ 0.49 \pm 0.01 $ & $ 0.50 \pm 0.00 $\\
$ d=18 $ & Time & $ \mathbf{ 14 \pm 0.29 } $ & $ 10,000 \pm 10 $ & $ 10,000 \pm 98 $\\\hline
\multirow{1}{*}{wXa} & Error & $ \mathbf{0.03 \pm 0.01} $ & $ 0.04 \pm 0.01 $ & $ \mathbf{ 0.03 \pm 0.01 } $\\
$ n=34,780 $ & NLL & $ 0.27 \pm 0.07 $ & $ 0.25 \pm 0.07 $ & $ \mathbf{ 0.19 \pm 0.06 } $\\
$ d=300 $ & Time & $ 66 \pm 16 $ & $ 612 \pm 11 $ & $ \mathbf{ 1.4 \pm 0.10 } $\\\hline
\end{tabular}
\end{adjustbox}
\caption{Average test prediction error, negative test log-likelihood (NLL) and time in seconds along with one standard deviation.
}
\label{tab:performance}
\end{table}


==> arXiv18_11 (AAAI version)/plot_inducing_points.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.7\textwidth]{Figures/ShuttleInducingPointsPlot.png}
\caption{Prediction error as function of training time (on a $\log_{10}$ scale) for the Shuttle dataset. Different numbers of inducing points are considered, $M = 16, 32, 64, 128$. X-GPC converges the fastest in all settings of different numbers of inducing points. Using only 32 inducing points is enought for obtaining allmost optimal prediction performance for all methods, but SVGPC becomes instable in settings of less than 128 inducing points.}
\label{fig:inducing_points}
\end{figure*}


==> arXiv18_11 (AAAI version)/plot_times.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.7\textwidth]{Figures/FinalConvergence_vs_time_on_Electricity.png}
\includegraphics[width=0.7\textwidth]{Figures/FinalConvergence_vs_time_on_Cod-rna.png}
\includegraphics[width=0.7\textwidth]{Figures/FinalConvergence_vs_time_on_SUSY.png}
\caption{Average median of the negative test log-likelihood and average test prediction error as a function of training time (seconds in a $\log_{10}$ scale) on the datasets Electricity (45,312 points), Cod RNA (343,564 points) and SUSY (5 million points).} 
\label{fig:timeexperiment}
\end{figure*}%

==> arXiv18_11 (AAAI version)/preamble_arXiv_compatible.tex <==
% FONTS
\usepackage[T1]{fontenc}

% Replace default Latin Modern typewriter with its proportional counterpart
% http://www.tug.dk/FontCatalogue/lmoderntypewriterprop/
\renewcommand*\ttdefault{lmvtt}

%%% OPTION 3 - MTPRO 2 Math + Termes Times + ParaType Sans

\usepackage{tgtermes}
\usepackage{amsmath}
%\usepackage[subscriptcorrection,
%            amssymbols,
%            mtpbb,
%            mtpcal,
%            nofontinfo  % suppresses all warnings
%           ]{mtpro2}
\usepackage{scalefnt,letltxmacro}
\LetLtxMacro{\oldtextsc}{\textsc}
\renewcommand{\textsc}[1]{\oldtextsc{\scalefont{1.10}#1}}
\usepackage[scaled=0.92]{PTSans}

% COLOR
\usepackage[usenames,dvipsnames]{xcolor}
\definecolor{shadecolor}{gray}{0.9}

% SPACING and TEXT
%\usepackage[final,expansion=alltext]{microtype} % DELETED!
\usepackage[english]{babel}
\usepackage[parfill]{parskip}
\usepackage{afterpage}
\usepackage{framed}
\usepackage{nicefrac}

% EDITING
% line numbering in left margin
\usepackage{lineno}
\renewcommand\linenumberfont{\normalfont
                             \footnotesize
                             \sffamily
                             \color{SkyBlue}}
% ragged paragraphs in right margin
\usepackage{ragged2e}
\DeclareRobustCommand{\sidenote}[1]{\marginpar{
                                    \RaggedRight
                                    \textcolor{Plum}{\textsf{#1}}}}
% paragraph helper
\DeclareRobustCommand{\PP}{\textcolor{Plum}{\P}~}
\DeclareRobustCommand{\pp}{\textcolor{Plum}{\P}~}
\DeclareRobustCommand{\parhead}[1]{\vspace{0.05in} \textbf{#1} }

% COUNTERS
\renewcommand{\labelenumi}{\color{black!67}{\arabic{enumi}.}}
\renewcommand{\labelenumii}{{\color{black!67}(\alph{enumii})}}
\renewcommand{\labelitemi}{{\color{black!67}\textbullet}}

% FIGURES
\usepackage{graphicx}
\usepackage[labelfont=bf]{caption}
%\usepackage[format=hang]{subcaption}
\usepackage{subfig}

% TABLES
\usepackage{booktabs}
\usepackage{tabu}

% BIBLIOGRAPHY
\usepackage{natbib}

% ALGORITHMS
%\usepackage[algoruled]{algorithm2e}
\usepackage{listings}
\usepackage{fancyvrb}
\fvset{fontsize=\normalsize}

% HYPERREF
\usepackage[colorlinks,linktoc=all]{hyperref}
\usepackage[all]{hypcap}
\hypersetup{citecolor=Violet}
\hypersetup{linkcolor=black}
\hypersetup{urlcolor=MidnightBlue}

% CLEVEREF must come after HYPERREF
\usepackage[nameinlink]{cleveref}

% ACRONYMS
\usepackage
[acronym,smallcaps,nowarn,section,nogroupskip,nonumberlist]{glossaries}
\glsdisablehyper{}
\crefname{appendix}{supplement}{}
% \makeglossaries

% COLOR DEFINITIONS
\newcommand{\red}[1]{\textcolor{BrickRed}{#1}}
\newcommand{\orange}[1]{\textcolor{BurntOrange}{#1}}
\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{MidnightBlue}{#1}}
\newcommand{\gray}[1]{\textcolor{black!60}{#1}}

% LISTINGS DEFINTIONS
\usepackage{listings}
\lstdefinestyle{alp_style}{
    commentstyle=\color{OliveGreen},
    numberstyle=\tiny\color{black!60},
    stringstyle=\color{BrickRed},
    basicstyle=\ttfamily\scriptsize,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=none,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}
\lstset{style=alp_style}

==> arXiv18_11 (AAAI version)/table.tex <==
\begin{table}[h!]\centering
	\begin{adjustbox}{max width=\columnwidth}
		\footnotesize
		\begin{tabular}{|l|l|l|l|l|}
			Dataset & & \textbf{X-GPC} (ours) & SVGPC & EPGPC \\\hline
			\multirow{1}{*}{aXa} & Error & $ 0.17 \pm 0.07 $ & $ 0.18 \pm 0.07 $ & $ \mathbf{ 0.16 \pm 0.07 } $\\
			$ n=36,974 $ & NLL & $ \mathbf{ 0.30 \pm 0.13 } $ & $ 0.37 \pm 0.13 $ & $ 0.34 \pm 0.13 $\\
			$ d=123 $ & Time & $ \mathbf{ 3.9 \pm 0.25 } $ & $ 10 \pm 0.54 $ & $ 673 \pm 7.6 $\\\hline
			\multirow{1}{*}{Bank Market.} & Error & $ 0.12 \pm 0.12 $ & $ 0.12 \pm 0.12 $ & $ \mathbf{ 0.11 \pm 0.13 } $\\
			$ n=45,211 $ & NLL & $ \mathbf{ 0.24 \pm 0.28 } $ & $ 0.32 \pm 0.26 $ & $ 0.32 \pm 0.19 $\\
			$ d=43 $ & Time & $ \mathbf{ 2.8 \pm 0.15 } $ & $ 10 \pm 0.51 $ & $ 4.2 \pm 0.28 $\\\hline
			\multirow{1}{*}{Click Pred.} & Error & $ \mathbf{ 0.17 \pm 0.00 } $ & $ \mathbf{0.17 \pm 0.01} $ & $ \mathbf{0.17 \pm 0.00} $\\
			$ n=399,482 $ & NLL & $ \mathbf{ 0.42 \pm 0.08 } $ & $ 0.47 \pm 0.01 $ & $ 0.46 \pm 0.01 $\\
			$ d=12 $ & Time & $ \mathbf{ 29 \pm 10 } $ & $ 119 \pm 13 $ & $ 63 \pm 15 $\\\hline
			\multirow{1}{*}{Cod RNA} & Error & $ \mathbf{ 0.05 \pm 0.00 } $ & $ 0.07 \pm 0.02 $ & $ \mathbf{0.05 \pm 0.00} $\\
			$ n=343,564 $ & NLL & $ \mathbf{ 0.15 \pm 0.04 } $ & $ 0.22 \pm 0.04 $ & $ 0.19 \pm 0.00 $\\
			$ d=8 $ & Time & $ \mathbf{ 13 \pm 0.46 } $ & $ 131 \pm 15 $ & $ 602 \pm 136 $\\\hline
			\multirow{1}{*}{Diabetes} & Error & $ \mathbf{ 0.23 \pm 0.06 } $ & $ \mathbf{0.23 \pm 0.07} $ & $ 0.24 \pm 0.06 $\\
			$ n=768 $ & NLL & $ 0.48 \pm 0.10 $ & $ \mathbf{ 0.47 \pm 0.10 } $ & $ 0.49 \pm 0.08 $\\
			$ d=8 $ & Time & $ 8.1 \pm 0.83 $ & $ 20 \pm 0.48 $ & $ \mathbf{ 0.56 \pm 0.31 } $\\\hline
			\multirow{1}{*}{Electricity} & Error & $ 0.27 \pm 0.07 $ & $ \mathbf{0.26 \pm 0.07}$ & $ \mathbf{ 0.26 \pm 0.06 } $\\
			$ n=45,312 $ & NLL & $ \mathbf{ 0.33 \pm 0.21 } $ & $ 0.54 \pm 0.09 $ & $ 0.53 \pm 0.05 $\\
			$ d=8 $ & Time & $ \mathbf{ 2.7 \pm 0.38 } $ & $ 9.8 \pm 0.36 $ & $ 3.7 \pm 0.25 $\\\hline
			\multirow{1}{*}{German} & Error & $ 0.25 \pm 0.12 $ & $ \mathbf{ 0.24 \pm 0.12 } $ & $ 0.25 \pm 0.11 $\\
			$ n=1,000 $ & NLL & $ \mathbf{ 0.44 \pm 0.16 } $ & $ 0.50 \pm 0.15 $ & $ 0.52 \pm 0.13 $\\
			$ d=20 $ & Time & $ 9.6 \pm 0.57 $ & $ 43 \pm 0.69 $ & $ \mathbf{ 3.8 \pm 0.57 } $\\\hline
			\multirow{1}{*}{Higgs} & Error & $ 0.37 \pm 0.01 $ & $ 0.45 \pm 0.01 $ & $ \mathbf{0.33 \pm 0.01} $\\
			$ n=11,000,000 $ & NLL & $ \mathbf{ 0.55 \pm 0.18 } $ & $ 0.69 \pm 0.00 $ & $ 0.66 \pm 0.00 $\\
			$ d=28 $ & Time & $ \mathbf{ 453 \pm 45 } $ & $ 1083 \pm 54 $ & $ 10,000 \pm 0 $\\\hline
			\multirow{1}{*}{IJCNN} & Error & $  0.07 \pm 0.01 $ & $ 0.09 \pm 0.01 $ & $\mathbf{ 0.04 \pm 0.01} $\\
			$ n=141,691 $ & NLL & $ 0.16 \pm 0.04 $ & $ 0.27 \pm 0.04 $ & $ \mathbf{ 0.08 \pm 0.04} $\\
			$ d=22 $ & Time & $ \mathbf{ 9.3 \pm 3.7 } $ & $ 74 \pm 8.1 $ & $ 10,000 \pm 0 $\\\hline
			% \multirow{1}{*}{Mnist} & Error & $ 0.20 \pm 0.02 $ & $ 0.26 \pm 0.13 $ & $ \mathbf{ 0.19 \pm 0.02 } $\\
			% $ n=70000 $ & NLL & $ \mathbf{ 0.35 \pm 0.13 } $ & $ 0.56 \pm 0.08 $ & $ 0.48 \pm 0.02 $\\
			% $ d=780 $ & Time & $ \mathbf{ 25 \pm 1.4 } $ & $ 76 \pm 32 $ & $ 122 \pm 8.2 $\\\hline
			\multirow{1}{*}{Shuttle} & Error & $ 0.02 \pm 0.01 $ & $ \mathbf{ 0.01 \pm 0.07 } $ & $ 0.02 \pm 0.01 $\\
			$ n=58,000 $ & NLL & $ 0.11 \pm 0.03 $ & $ \mathbf{ 0.07 \pm 0.43 } $ & $ 0.07 \pm 0.01 $\\
			$ d=9 $ & Time & $ \mathbf{ 1.0 \pm 0.24 } $ & $ 9.3 \pm 0.35 $ & $ 63 \pm 1.4 $\\\hline
			\multirow{1}{*}{SUSY} & Error & $ \mathbf{ 0.22 \pm 0.00 } $ & $ 0.23 \pm 0.01 $ & $ 0.23 \pm 0.00 $\\
			$ n=5,000,000 $ & NLL & $ 0.54 \pm 0.15 $ & $ 0.53 \pm 0.01 $ & $ \mathbf{ 0.51 \pm 0.00 } $\\
			$ d=18 $ & Time & $ \mathbf{ 275 \pm 152 } $ & $ 469 \pm 47 $ & $ 1886 \pm 194 $\\\hline
			\multirow{1}{*}{wXa} & Error & $ \mathbf{0.02 \pm 0.01} $ & $ \mathbf{ 0.02 \pm 0.01 } $ & $ 0.03 \pm 0.01 $\\
			$ n=34,780 $ & NLL & $ \mathbf{ 0.14 \pm 0.09 } $ & $ 0.33 \pm 0.07 $ & $ 0.21 \pm 0.11 $\\
			$ d=300 $ & Time & $ 8.0 \pm 0.64 $ & $ 18 \pm 0.93 $ & $ \mathbf{ 5.4 \pm 0.32 } $\\\hline
			\end{tabular}
	\end{adjustbox}
	\caption{Average test prediction error, negative test log-likelihood (NLL) and time in seconds along with one standard deviation. For the datasets IJCNN and Higgs, EPGPC exceeded the time budget of $10^5$ seconds ($\approx$ 28h).
	}
	\label{tab:performance}
\end{table}


==> new_table.tex <==
\begin{table}[h!]\centering
\begin{adjustbox}{max width=\columnwidth}
\footnotesize
\begin{tabular}{|l|l|l|l|l|}
Dataset & & \textbf{X-GPC} & SVGPC & EPGPC \\\hline
\multirow{1}{*}{aXa} & Error & $ \mathbf{0.17 \pm 0.07} $ & $ \mathbf{0.17 \pm 0.07} $ & $ \mathbf{ 0.17 \pm 0.07 } $\\
$ n=36,974 $ & NLL & $ \mathbf{ 0.29 \pm 0.13 } $ & $ 0.36 \pm 0.13 $ & $ 0.34 \pm 0.13 $\\
$ d=123 $ & Time & $ \mathbf{ 47 \pm 2.2 } $ & $ 451 \pm 7.8 $ & $ 214 \pm 4.8 $\\\hline
\multirow{1}{*}{Bank Market.} & Error & $ 0.14 \pm 0.12 $ & $ \mathbf{0.12 \pm 0.12} $ & $ \mathbf{ 0.12 \pm 0.13 } $\\
$ n=45,211 $ & NLL & $ \mathbf{ 0.27 \pm 0.22 } $ & $ 0.31 \pm 0.26 $ & $ 0.33 \pm 0.20 $\\
$ d=43 $ & Time & $ \mathbf{ 9 \pm 1.5 } $ & $ 205 \pm 6.6 $ & $ 46 \pm 3.5 $\\\hline
\multirow{1}{*}{Click Pred.} & Error & $ \mathbf{ 0.17 \pm 0.00 } $ & $ \mathbf{0.17 \pm 0.00} $ & $ \mathbf{0.17 \pm 0.01} $\\
$ n=399,482 $ & NLL & $ \mathbf{ 0.39 \pm 0.07 } $ & $ 0.46 \pm 0.00 $ & $ 0.46 \pm 0.01 $\\
$ d=12 $ & Time & $ \mathbf{4.5 \pm 1.3} $ & $ 102 \pm 3.0 $ & $ 8.1 \pm 0.45 $\\\hline
\multirow{1}{*}{Cod RNA} & Error & $ \mathbf{ 0.04 \pm 0.00 } $ & $ \mathbf{0.04 \pm 0.00} $ & $ \mathbf{0.04 \pm 0.00} $\\
$ n=343,564 $ & NLL & $ \mathbf{ 0.11 \pm 0.03 } $ & $ 0.13 \pm 0.00 $ & $ 0.12 \pm 0.00 $\\
$ d=8 $ & Time & $ \mathbf{ 3.7 \pm 0.13 } $ & $ 115 \pm 4.3 $ & $ 869 \pm 5.2 $\\\hline
\multirow{1}{*}{Diabetes} & Error & $ \mathbf{0.23 \pm 0.07} $ & $ \mathbf{ 0.23 \pm 0.06 } $ & $ 0.24 \pm 0.06 $\\
$ n=768 $ & NLL & $ \mathbf{ 0.47 \pm 0.11 } $ & $ 0.47 \pm 0.10 $ & $ 0.48 \pm 0.09 $\\
$ d=8 $ & Time & $ 8.8 \pm 0.12 $ & $ 150 \pm 5.1 $ & $ \mathbf{ 8 \pm 0.45 } $\\\hline
\multirow{1}{*}{Electricity} & Error & $ \mathbf{ 0.24 \pm 0.06 } $ & $ 0.26 \pm 0.06 $ & $ 0.26 \pm 0.06 $\\
$ n=45,312 $ & NLL & $ \mathbf{ 0.31 \pm 0.17 } $ & $ 0.53 \pm 0.08 $ & $ 0.53 \pm 0.06 $\\
$ d=8 $ & Time & $ \mathbf{8.2 \pm 0.48} $ & $ 356 \pm 6.9 $ & $ 13.5 \pm 1.50 $\\\hline
\multirow{1}{*}{German} & Error & $ \mathbf{0.25 \pm 0.12} $ & $ \mathbf{ 0.25 \pm 0.11 } $ & $ 0.26 \pm 0.13 $\\
$ n=1,000 $ & NLL & $ \mathbf{ 0.44 \pm 0.17 } $ & $ 0.51 \pm 0.15 $ & $ 0.53 \pm 0.11 $\\
$ d=20 $ & Time & $ 17 \pm 0.42 $ & $ 374 \pm 7.3 $ & $ \mathbf{ 5.2 \pm 0.03 } $\\\hline
\multirow{1}{*}{Higgs} & Error & $ \mathbf{ 0.33 \pm 0.01 } $ & $ 0.45 \pm 0.01 $ & $ 0.38 \pm 0.01 $\\
$ n=11,000,000 $ & NLL & $ \mathbf{ 0.55 \pm 0.13 } $ & $ 0.69 \pm 0.00 $ & $ 0.66 \pm 0.00 $\\
$ d=28 $ & Time & $ \mathbf{ 23 \pm 0.88 } $ & $ 294 \pm 54 $ & $ 8732 \pm 867 $\\\hline
\multirow{1}{*}{IJCNN} & Error & $ 0.03 \pm 0.01 $ & $ 0.06 \pm 0.01 $ & $\mathbf{ 0.02 \pm 0.01} $\\
$ n=141,691 $ & NLL & $ 0.10 \pm 0.03 $ & $ 0.15 \pm 0.07 $ & $ \mathbf{0.09 \pm 0.04} $\\
$ d=22 $ & Time & $ \mathbf{17 \pm 0.44} $ & $ 1033 \pm 45 $ & $ 756 \pm 8.6 $\\\hline
\multirow{1}{*}{Mnist} & Error & $  0.14 \pm 0.01  $ & $ 0.44 \pm 0.13 $ & $ \mathbf{0.12\pm 0.01} $\\
$ n=70,000 $ & NLL & $ \mathbf{ 0.24 \pm 0.10 } $ & $ 0.66 \pm 0.11 $ & $ 0.27 \pm 0.01 $\\
$ d=780 $ & Time & $ \mathbf{200 \pm 5.5} $ & $ 991 \pm 23 $ & $ 806 \pm 5.2 $\\\hline
\multirow{1}{*}{Shuttle} & Error & $ \mathbf{ 0.01 \pm 0.01 } $ & $ \mathbf{0.01 \pm 0.00} $ & $ \mathbf{0.01 \pm 0.01} $\\
$ n=58,000 $ & NLL & $ \mathbf{ 0.07 \pm 0.01 } $ & $ \mathbf{0.07 \pm 0.00} $ & $\mathbf{ 0.07 \pm 0.01 }$\\
$ d=9 $ & Time & $ \mathbf{ 0.01 \pm 0.00 } $ & $ 7.5 \pm 0.7 $ & $ 100 \pm 0.63 $\\\hline
\multirow{1}{*}{SUSY} & Error & $ \mathbf{ 0.21 \pm 0.00 } $ & $ 0.22 \pm 0.00 $ & $ 0.22 \pm 0.00 $\\
$ n=5,000,000 $ & NLL & $ \mathbf{ 0.31 \pm 0.10 } $ & $ 0.49 \pm 0.01 $ & $ 0.50 \pm 0.00 $\\
$ d=18 $ & Time & $ \mathbf{ 14 \pm 0.29 } $ & $ 10,000 \pm 10 $ & $ 10,000 \pm 98 $\\\hline
\multirow{1}{*}{wXa} & Error & $ \mathbf{0.03 \pm 0.01} $ & $ 0.04 \pm 0.01 $ & $ \mathbf{ 0.03 \pm 0.01 } $\\
$ n=34,780 $ & NLL & $ 0.27 \pm 0.07 $ & $ 0.25 \pm 0.07 $ & $ \mathbf{ 0.19 \pm 0.06 } $\\
$ d=300 $ & Time & $ 66 \pm 16 $ & $ 612 \pm 11 $ & $ \mathbf{ 1.4 \pm 0.10 } $\\\hline
\end{tabular}
\end{adjustbox}
\caption{Average test prediction error, negative test log-likelihood (NLL) and time in seconds along with one standard deviation.
}
\label{tab:performance}
\end{table}


==> plot_inducing_points.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.7\textwidth]{Figures/ShuttleInducingPointsPlot.png}
\caption{Prediction error as function of training time (on a $\log_{10}$ scale) for the Shuttle dataset. Different numbers of inducing points are considered, $M = 16, 32, 64, 128$. X-GPC converges the fastest in all settings of different numbers of inducing points. Using only 32 inducing points is enought for obtaining allmost optimal prediction performance for all methods, but SVGPC becomes instable in settings of less than 128 inducing points.}
\label{fig:inducing_points}
\end{figure*}


==> plot_times.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.7\textwidth]{Figures/FinalConvergence_vs_time_on_Electricity.png}
\includegraphics[width=0.7\textwidth]{Figures/FinalConvergence_vs_time_on_Cod-rna.png}
\includegraphics[width=0.7\textwidth]{Figures/FinalConvergence_vs_time_on_SUSY.png}
\caption{Average median of the negative test log-likelihood and average test prediction error as a function of training time (seconds in a $\log_{10}$ scale) on the datasets Electricity (45,312 points), Cod RNA (343,564 points) and SUSY (5 million points).} 
\label{fig:timeexperiment}
\end{figure*}%

==> table.tex <==
\begin{table}[h!]\centering
	\begin{adjustbox}{max width=\columnwidth}
		\footnotesize
		\begin{tabular}{|l|l|l|l|l|}
			Dataset & & \textbf{X-GPC} (ours) & SVGPC & EPGPC \\\hline
			\multirow{1}{*}{aXa} & Error & $ 0.17 \pm 0.07 $ & $ 0.18 \pm 0.07 $ & $ \mathbf{ 0.16 \pm 0.07 } $\\
			$ n=36,974 $ & NLL & $ \mathbf{ 0.30 \pm 0.13 } $ & $ 0.37 \pm 0.13 $ & $ 0.34 \pm 0.13 $\\
			$ d=123 $ & Time & $ \mathbf{ 3.9 \pm 0.25 } $ & $ 10 \pm 0.54 $ & $ 673 \pm 7.6 $\\\hline
			\multirow{1}{*}{Bank Market.} & Error & $ 0.12 \pm 0.12 $ & $ 0.12 \pm 0.12 $ & $ \mathbf{ 0.11 \pm 0.13 } $\\
			$ n=45,211 $ & NLL & $ \mathbf{ 0.24 \pm 0.28 } $ & $ 0.32 \pm 0.26 $ & $ 0.32 \pm 0.19 $\\
			$ d=43 $ & Time & $ \mathbf{ 2.8 \pm 0.15 } $ & $ 10 \pm 0.51 $ & $ 4.2 \pm 0.28 $\\\hline
			\multirow{1}{*}{Click Pred.} & Error & $ \mathbf{ 0.17 \pm 0.00 } $ & $ \mathbf{0.17 \pm 0.01} $ & $ \mathbf{0.17 \pm 0.00} $\\
			$ n=399,482 $ & NLL & $ \mathbf{ 0.42 \pm 0.08 } $ & $ 0.47 \pm 0.01 $ & $ 0.46 \pm 0.01 $\\
			$ d=12 $ & Time & $ \mathbf{ 29 \pm 10 } $ & $ 119 \pm 13 $ & $ 63 \pm 15 $\\\hline
			\multirow{1}{*}{Cod RNA} & Error & $ \mathbf{ 0.05 \pm 0.00 } $ & $ 0.07 \pm 0.02 $ & $ \mathbf{0.05 \pm 0.00} $\\
			$ n=343,564 $ & NLL & $ \mathbf{ 0.15 \pm 0.04 } $ & $ 0.22 \pm 0.04 $ & $ 0.19 \pm 0.00 $\\
			$ d=8 $ & Time & $ \mathbf{ 13 \pm 0.46 } $ & $ 131 \pm 15 $ & $ 602 \pm 136 $\\\hline
			\multirow{1}{*}{Diabetes} & Error & $ \mathbf{ 0.23 \pm 0.06 } $ & $ \mathbf{0.23 \pm 0.07} $ & $ 0.24 \pm 0.06 $\\
			$ n=768 $ & NLL & $ 0.48 \pm 0.10 $ & $ \mathbf{ 0.47 \pm 0.10 } $ & $ 0.49 \pm 0.08 $\\
			$ d=8 $ & Time & $ 8.1 \pm 0.83 $ & $ 20 \pm 0.48 $ & $ \mathbf{ 0.56 \pm 0.31 } $\\\hline
			\multirow{1}{*}{Electricity} & Error & $ 0.27 \pm 0.07 $ & $ \mathbf{0.26 \pm 0.07}$ & $ \mathbf{ 0.26 \pm 0.06 } $\\
			$ n=45,312 $ & NLL & $ \mathbf{ 0.33 \pm 0.21 } $ & $ 0.54 \pm 0.09 $ & $ 0.53 \pm 0.05 $\\
			$ d=8 $ & Time & $ \mathbf{ 2.7 \pm 0.38 } $ & $ 9.8 \pm 0.36 $ & $ 3.7 \pm 0.25 $\\\hline
			\multirow{1}{*}{German} & Error & $ 0.25 \pm 0.12 $ & $ \mathbf{ 0.24 \pm 0.12 } $ & $ 0.25 \pm 0.11 $\\
			$ n=1,000 $ & NLL & $ \mathbf{ 0.44 \pm 0.16 } $ & $ 0.50 \pm 0.15 $ & $ 0.52 \pm 0.13 $\\
			$ d=20 $ & Time & $ 9.6 \pm 0.57 $ & $ 43 \pm 0.69 $ & $ \mathbf{ 3.8 \pm 0.57 } $\\\hline
			\multirow{1}{*}{Higgs} & Error & $ 0.37 \pm 0.01 $ & $ 0.45 \pm 0.01 $ & $ \mathbf{0.33 \pm 0.01} $\\
			$ n=11,000,000 $ & NLL & $ \mathbf{ 0.55 \pm 0.18 } $ & $ 0.69 \pm 0.00 $ & $ 0.66 \pm 0.00 $\\
			$ d=28 $ & Time & $ \mathbf{ 453 \pm 45 } $ & $ 1083 \pm 54 $ & $ 10,000 \pm 0 $\\\hline
			\multirow{1}{*}{IJCNN} & Error & $  0.07 \pm 0.01 $ & $ 0.09 \pm 0.01 $ & $\mathbf{ 0.04 \pm 0.01} $\\
			$ n=141,691 $ & NLL & $ 0.16 \pm 0.04 $ & $ 0.27 \pm 0.04 $ & $ \mathbf{ 0.08 \pm 0.04} $\\
			$ d=22 $ & Time & $ \mathbf{ 9.3 \pm 3.7 } $ & $ 74 \pm 8.1 $ & $ 10,000 \pm 0 $\\\hline
			% \multirow{1}{*}{Mnist} & Error & $ 0.20 \pm 0.02 $ & $ 0.26 \pm 0.13 $ & $ \mathbf{ 0.19 \pm 0.02 } $\\
			% $ n=70000 $ & NLL & $ \mathbf{ 0.35 \pm 0.13 } $ & $ 0.56 \pm 0.08 $ & $ 0.48 \pm 0.02 $\\
			% $ d=780 $ & Time & $ \mathbf{ 25 \pm 1.4 } $ & $ 76 \pm 32 $ & $ 122 \pm 8.2 $\\\hline
			\multirow{1}{*}{Shuttle} & Error & $ 0.02 \pm 0.01 $ & $ \mathbf{ 0.01 \pm 0.07 } $ & $ 0.02 \pm 0.01 $\\
			$ n=58,000 $ & NLL & $ 0.11 \pm 0.03 $ & $ \mathbf{ 0.07 \pm 0.43 } $ & $ 0.07 \pm 0.01 $\\
			$ d=9 $ & Time & $ \mathbf{ 1.0 \pm 0.24 } $ & $ 9.3 \pm 0.35 $ & $ 63 \pm 1.4 $\\\hline
			\multirow{1}{*}{SUSY} & Error & $ \mathbf{ 0.22 \pm 0.00 } $ & $ 0.23 \pm 0.01 $ & $ 0.23 \pm 0.00 $\\
			$ n=5,000,000 $ & NLL & $ 0.54 \pm 0.15 $ & $ 0.53 \pm 0.01 $ & $ \mathbf{ 0.51 \pm 0.00 } $\\
			$ d=18 $ & Time & $ \mathbf{ 275 \pm 152 } $ & $ 469 \pm 47 $ & $ 1886 \pm 194 $\\\hline
			\multirow{1}{*}{wXa} & Error & $ \mathbf{0.02 \pm 0.01} $ & $ \mathbf{ 0.02 \pm 0.01 } $ & $ 0.03 \pm 0.01 $\\
			$ n=34,780 $ & NLL & $ \mathbf{ 0.14 \pm 0.09 } $ & $ 0.33 \pm 0.07 $ & $ 0.21 \pm 0.11 $\\
			$ d=300 $ & Time & $ 8.0 \pm 0.64 $ & $ 18 \pm 0.93 $ & $ \mathbf{ 5.4 \pm 0.32 } $\\\hline
			\end{tabular}
	\end{adjustbox}
	\caption{Average test prediction error, negative test log-likelihood (NLL) and time in seconds along with one standard deviation. For the datasets IJCNN and Higgs, EPGPC exceeded the time budget of $10^5$ seconds ($\approx$ 28h).
	}
	\label{tab:performance}
\end{table}

